LUCID: A Practical, Lightweight Deep Learning Solution for DDoS Attack Detection

Distributed Denial of Service (DDoS) attacks are one of the most harmful threats in today's Internet, disrupting the availability of essential services. The challenge of DDoS detection is the combination of attack approaches coupled with the volume of live traffic to be analysed. In this paper, we present a practical, lightweight deep learning DDoS detection system called LUCID, which exploits the properties of Convolutional Neural Networks (CNNs) to classify traffic flows as either malicious or benign. We make four main contributions; (1) an innovative application of a CNN to detect DDoS traffic with low processing overhead, (2) a dataset-agnostic preprocessing mechanism to produce traffic observations for online attack detection, (3) an activation analysis to explain LUCID's DDoS classification, and (4) an empirical validation of the solution on a resource-constrained hardware platform. Using the latest datasets, LUCID matches existing state-of-the-art detection accuracy whilst presenting a 40x reduction in processing time, as compared to the state-of-the-art. With our evaluation results, we prove that the proposed approach is suitable for effective DDoS detection in resource-constrained operational environments.

==> background.tex <==
\section{Background}
\subsection{Artificial Neural Networks}
\textit{Introduction to ANNs (with some details related to CNNs and RNNs) and their benefits in anomaly/DDoS detection.}
\subsection{Datasets}\label{sec:datasets}
Our deep learning model has been validated with recent datasets ISCXIDS2012 \cite{ISCXIDS2012}, CICIDS2017 \cite{CICIDS2017} and CSECICIDS2018 \cite{CSECICIDS2018} provided by the Canadian Institute for Cybersecurity of the \ac{unb}, Canada. They consist of several days of network activity, normal and malicious, including \ac{ddos} attacks. The three datasets are publicly available in form traffic traces in \textit{pcap} format including full packet payloads, plus supplementary text files containing the labels and statistical details for each traffic flow. 

The \ac{unb} researchers have generated these datasets by using profiles to accurately represent the abstract properties of human and attack behaviours. One profile characterises the normal network activities and provides distribution models for applications and  protocols (HTTP, SMTP, SSH, IMAP, POP3, and FTP) produced with the analysis of real traffic traces. Other profiles describe a variety of attack scenarios based on recent security reports. They are used to mimic the behaviour of the malicious attackers by means of custom botnets and well-known \ac{ddos} attacking tools such as High Orbit Ion Cannon (HOIC)~\cite{hoic} and its predecessor, the Low Orbit Ion Cannon (LOIC)~\cite{loic}. HOIC and LOIC has been widely used by Anonymous and other hacker groups in some highly-publicized attacks against PayPal, Mastercard, Visa, Amazon, Megaupload, among others.

Table \ref{tab:datasets} shows the parts of the three datasets used in this work. In the table, the column \textit{Traffic trace} specifies the name of the trace, according to \cite{ISCXIDS2012}, \cite{CICIDS2017} and \cite{CSECICIDS2018}. With respect to the original file, the trace \textit{Fri7PM} has been reduced to timeslot 3.30PM-5.00PM to exclude malicious packets related to other cyber attacks (port scans and backdoors). 
However, as this results in a limited number of benign flows for dataset CICIDS2017, flows from trace \textit{Mon3} has been used for balancing without losing precious malicious flows, as described in Section \ref{sec:features}. 

\begin{table}[h!]
	\caption{The datasets used for the evaluation.} 
	\label{tab:datasets}
	\small % text size of table content
	\centering % center the table
	\begin{tabular}{llccc} \toprule[\heavyrulewidth]
		\textbf{Dataset} & \textbf{Traffic trace} & \textbf{\#Flows} & \textbf{\#Benign} & \textbf{\#Attack} \\ \midrule[\heavyrulewidth]
		ISCXIDS2012	& Tue15 & 571698 & 534320 & 37378\\ \midrule
		\multirow{2}*{CICIDS2017}  
		& Mon3 & 529518 & 529518 & 0 \\ 
		& Fri7PM & 225745 & 97718 & 128027 \\ \midrule
		CSECICIDS2018& Wed21 & 1048575 & 360832 & 687743\\ \bottomrule[\heavyrulewidth]
	\end{tabular}
\end{table}

